Search for direct production of charginos and neutralinos in events with three leptons and missing transverse momentum in sqrt(s) = 8TeV pp collisions with the ATLAS detector

A search for the direct production of charginos and neutralinos in final states with three leptons and missing transverse momentum is presented. The analysis is based on 20.3 fb-1 of sqrt(s) = 8 TeV proton--proton collision data delivered by the Large Hadron Collider and recorded with the ATLAS detector. Observations are consistent with the Standard Model expectations and limits are set in R-parity-conserving phenomenological Minimal Supersymmetric Standard Models and in simplified supersymmetric models, significantly extending previous results. For simplified supersymmetric models of direct chargino ($\tilde\chi^\pm_1$) and next-to-lightest neutralino ($\tilde{\chi}_2^0$) production with decays to lightest neutralino ($\tilde{\chi}_1^0$) via either all three generations of sleptons, staus only, gauge bosons, or Higgs bosons, $\tilde\chi^\pm_1$ and $\tilde{\chi}_2^0$ masses are excluded up to 700 GeV, 380 GeV, 345 GeV, or 148 GeV respectively, for a massless $\tilde{\chi}_1^0$.

==> numbers.tex <==
\newcommand{\integLumi}{\unit[2]{\ifb}\xspace}
\newcommand{\integLumiE}{\unit[$(2.05\pm 0.08)$]{\ifb}\xspace}
\newcommand{\nDatalowpt}{6\xspace}
\newcommand{\nData}{3\xspace}
% \newcommand{\nBackground}{\ensuremath{7.23\pm1.56\pm1.25}\xspace}
\newcommand{\nBackgroundlowpt}{\ensuremath{7.23\pm1.56\pm1.61}\xspace}
\newcommand{\nBackground}{\ensuremath{5.3\pm1.3\pm2.2}\xspace}
\newcommand{\nGMSBBenchmark}{\ensuremath{20.8\pm3.4\pm5.4}\xspace}
\newcommand{\NCLs}{\ensuremath{5.6}\xspace}
\newcommand{\sigmaGMSBCLs}{\ensuremath{\sigma < \unit[(3-25)]{fb}}\xspace}
\newcommand{\GMSBLimitBestCLs}{\unit[47]{TeV}\xspace}
\newcommand{\GMSBLimitBestTanBetaCLs}{37\xspace}
\newcommand{\GMSBLimitCLs}{\unit[32]{TeV}\xspace}

